LMMs-Eval: Reality Check on the Evaluation of Large Multimodal Models

The advances of large foundation models necessitate wide-coverage, low-cost, and zero-contamination benchmarks. Despite continuous exploration of language model evaluations, comprehensive studies on the evaluation of Large Multi-modal Models (LMMs) remain limited. In this work, we introduce LMMS-EVAL, a unified and standardized multimodal benchmark framework with over 50 tasks and more than 10 models to promote transparent and reproducible evaluations. Although LMMS-EVAL offers comprehensive coverage, we find it still falls short in achieving low cost and zero contamination. To approach this evaluation trilemma, we further introduce LMMS-EVAL LITE, a pruned evaluation toolkit that emphasizes both coverage and efficiency. Additionally, we present Multimodal LIVEBENCH that utilizes continuously updating news and online forums to assess models' generalization abilities in the wild, featuring a low-cost and zero-contamination evaluation approach. In summary, our work highlights the importance of considering the evaluation trilemma and provides practical solutions to navigate the trade-offs in evaluating large multi-modal models, paving the way for more effective and reliable benchmarking of LMMs. We opensource our codebase and maintain leaderboard of LIVEBENCH at https://github.com/EvolvingLMMs-Lab/lmms-eval and https://huggingface.co/spaces/lmms-lab/LiveBench.

==> sections/evaluation_methods.tex <==
\section{Evaluation methods}

\subsection{Data Decontamination}

To illustrate our contamination method, we utilize the pretraining dataset and supervised fine-tuning data from \citet{liu2024llavanext}. We construct two different versions of the supervised fine-tuning data: one with user data and the other without any user data. 

\paragraph{Text overlap} To quantify text overlap, we employ an approach similar to that of GPT-4 \citep{openai2024gpt4}, PaLM \citep{anil2023palm}, and LLaMA \citep{touvron2023llama}, which relies on string matching. \citet{brown2020language} uses a range of 8-13 n-grams for different dataset, while we use 8 n-grams for simplicity. To mitigate the inclusion of meaningless n-gram overlap results, we disregard cases of overlap detected more than 10 times in the training data, adding them to a set of meaningless n-grams. Additionally, we compute an overlap ratio between each new possible n-gram candidate and the n-grams in the meaningless n-grams set and exclude those exceeding a certain threshold.

\paragraph{Image overlap} Contrary to text overlap, determining image overlap is a more challenging task. While it is common practice to compute image embeddings and then calculate their cosine similarity, selecting an appropriate threshold applicable to all datasets is difficult. Moreover, interpreting the significance of the chosen threshold can be hard. Instead of computing similarity in the embedding space, we empirically find that using the pretrained SEED-tokenizer leads to meaningful separation in detecting the overlap. We tokenize each image into a 1-D sequence of 32 tokens. Similar to text, an 8-gram lookup table was constructed from those image tokens to detect image contamination. The occurrence of 8-gram overlap can be interpreted as approximately 1/4 of the image overlapping.

\begin{comment}
\subsection{Sensitivity for benchmarks}

One aspect we aim to review in the current benchmark is the necessity of all questions for assessing the overall ability of the model. We question whether there may be redundant questions that could be excluded from the benchmark. If the benchmark's testing abilities remain unaffected even after removing most of the questions, we consider it to be insensitive to the removal of data points. Utilizing a subset of selected data points would then sufficient to cover the majority of testing cases.

Let the benchmark be represented as \(D = \{ (x_{i}, y_{i}) \}_{i=1}^{n}\) and the scoring function underlying the benchmark system be denoted as \(S\). Given a model \(f\), let the response of the model to a particular question in the dataset be denoted as \(f(x_{i}) = \widehat{y}_{i}\). We aim to select a subset of the benchmark \(V \in D\) such that

\begin{align}
    \label{eq:target_fun} &
    \frac{1}{\left | V \right |}\sum_{i=1}^{\left | V \right |}S(y_{i}, \widehat{y}_{i}) \approx \frac{1}{\left | D \right |}\sum_{i=1}^{\left | D \right |}S(y_{i}, \widehat{y}_{i})\ 
\end{align}

To attain this objective, we frame our task as a specific case of active learning \citep{mirzasoleiman2020coresets, yang2023sustainable, sener2018active} where we select \(N\) samples in each iteration without labeled data. By regarding the scoring function of the benchmark system as a special loss function, our aim transforms into an active learning problem, wherein we aim to minimize the loss between the subset and the entire dataset.

\begin{align}
    \label{eq:min_loss} &
    \min_{V:\left | V \right | \leq \left | D \right |} \left | \frac{1}{\left | D \right |} \sum_{i=1}^{\left | D \right |} S(y_{i}, \widehat{y}_{i}) -  \frac{1}{\left | V \right |} \sum_{i=1}^{\left | V \right |} S(y_{i}, \widehat{y}_{i}) \right |
\end{align}

\makebox[\textwidth][c]{
\begin{minipage}{0.8\textwidth}
\vspace{-2mm}
   \begin{algorithm}[H] 
   \caption{k-Center-Greedy} 
   \label{alg:greedy} 
   \begin{algorithmic}
        \State {\bfseries Input:} data $\mathbf{x}_i$ and $\left | V \right | = n$
        \State Initialize $\mathbf{s}=\mathbf{\phi}$
        \While{$\left | s \right | < n$}
            \State $u=\arg\max_{i \in D \setminus \mathbf{s}} \min_{j \in \mathbf{s}} \Delta(\mathbf{x}_i, \mathbf{x}_j)$ 
            \State $\mathbf{s} = \mathbf{s} \cup \{u\}$ 
        \EndWhile
        \State {\bfseries return} $\mathbf{s}$
\end{algorithmic}
\end{algorithm} 
\vspace{-3mm}
\end{minipage} 
}

It has been proved by \citet{sener2018active} that finding the subset \(V\) capable of minimizing the above target function is equivalent to solving the k-Center problem. The k-Center problem can be defined as follows: selecting b center points such that the maximum distance between a data point and its nearest center is minimized. Formally, we aim to solve:

\begin{align}
    \min_{V:\left | V \right | \leq \left | D \right |} \max_{i} \min_{j\in V} \Delta (x_{i}, x_{j})
\end{align}

Where \(x_{i}\) represents the embedding generated by the model \(f\). In contrast to \citet{sener2018active}, who employed image features extracted by the CNN for k-center clustering, we opted to utilize embeddings extracted from the final layer of the transformer model for clustering purposes.

However, \citet{cook1997combinatorial} have proven that finding the exact solution to the k-Center problem is NP-hard. Consequently, we choose to use a greedy algorithm, as outlined in Algorithm \ref{alg:greedy}, to efficiently compute the results. The greedy algorithm is capable of achieving a \(2\)-OPT solution.
\end{comment}

\subsection{LiveBench : an uncontaminated evaluation set}

\blindtext

==> sections/reference.tex <==



\bibliographystyle{plain}
\bibliography{citation}



==> tables/accessible_dataset.tex <==
% \renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{2pt}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}l|l|l|l|l|l|l@{}}
% \toprule
% \textbf{Datasets} & \textbf{Sources} & \textbf{Task Domains} & \textbf{Ground-Truth Types} & \textbf{Instances} & \textbf{Splits} & \textbf{Eval. Metrics} \\ \midrule
% AI2D \citep{kembhavi2016diagram} & Internet & Science,Diagram & Muiti-Choice & 3088 & test & Exact Match \\
% BenchLMM ~\citep{cai2023benchlmm} & Internet & Cross Style Understanding & Short Answer & Muiti-Choice &  &  &  \\
% ChartQA \citep{masry2022chartqa} & Internet & Chart & Short Answer & 2500 & test & Exact Match \\
% CMMMU \citep{zhang2024cmmmu} & Books & Internet & Multi-task,World Knowledge & Free-form & Muiti-Choice & 900/11000 & val/test & Accuracy \\
% COCO 2014 Caption \citep{lin2014microsoft} & COCO \citep{lin2014microsoft} & Captioning & Short Answer & 40775 / 40504 & test / val & Bleu / ROUGE_L / CIDEr \\
% COCO 2017 Caption \citep{lin2014microsoft} & MSCOCO \citep{lin2014microsoft} & Captioning & Short Answer & 40670 / 5000 & test / val & Bleu / ROUGE_L / CIDEr \\
% DocVQA \citep{mathew2020docvqa} & UCSF Industry Document Library & Document & Short Answer & 5349 & test & ANLS \\
% Ferret \citep{you2023ferret} & MSCOCO \citep{lin2014microsoft} & Referring or Grounding Actions & Free-form Answer & 120 & test & GPT4 Eval \\
% Flickr30k \citep{young2014image} & Flickr & Visual Understanding & Captioning & 31783 & test & Bleu / ROUGE_L / CIDEr \\
% GQA \citep{hudson2019gqa} & MSCOCO \citep{lin2014microsoft} & Flickr \citep{thomee2016yfcc100m} & Real-World Visual Reasoning & Compositional Question Answering & Short Answer & 12578 & test / dev & Exact Match \\
% Hallusion-Bench \citep{guan2023hallusionbench} & Original & Human-Modified & Multimodal Image-Context Reasoning & Yes or No & 951 & image & Accuracy \\
% IconQA \citep{lu2022iconqa} & Online (IXL Math Learning) & Abstract Diagrams & Muiti-Choice & Short Answer & 21489 / 21488 & test / val & ANLS \\
% InfoVQA \citep{Mathew_2022_WACV} & Internet & Infographics understanding & Extractive & Numerical & 2801 & val & ANLS \\
% LLaVA-COCO \citep{liu2023visual} & MSCOCO \citep{lin2014microsoft} & Conversation, Reasoning & Free-form Answer & 90 & test & GPT4 Eval \\
% LLaVA-W \citep{liu2023visual} & Internet & Conversation, Reasoning & Free-form Answer & 60 & test & GPT4 Eval \\
% LLaVA-Wilder \citep{liu2024llava} & Internet & User Requests & Conversation, Reasoning & Free-form Answer & 210/1020 & test & GPT4V Eval \\
% LiveBench (Ours) & Internet & Webpage Understanding & Lively Updated & Free-form & dynamic & test & GPT4V/Gemini/Claude Eval \\
% MathVista \citep{lu2024mathvista} & Internet & Mathematical Reasoning, Visual Understanding & Free-form & Muiti-Choice & 1000 & testmini & GPT4 Eval \\
% MathVerse \citep{zhang2024mathverse} & Internet & Mathematical Reasoning, Visual Understanding & Free-form & Muiti-Choice & 3940 & testmini & GPT4 Eval \\
% MMBench \citep{liu2023mmbench} & Internet & Public Dataset & Reasoning & Perception & Muiti-Choice & 6666 / 4329 & test / dev & GPT4 Eval \\
% MME \citep{fu2024mme} & MSCOCO \citep{lin2014microsoft} & Self-Collected & Perception, Cognition & Yes or No & 2374 & test & Exact Match \\
% MMMU \citep{yue2023mmmu} & Books & Internet & Multi-task,World Knowledge & Free-form & Muiti-Choice & 10500 / 900 & test / val & Accuracy \\
% MM-Vet \citep{yu2023mmvet} & Internet & Multi-task & Free-form & 218 & test & GPT4 Eval \\
% Multilingual-LLaVA-W & Internet & Multi-lingual Conversation,Reasoning & Free-form Answer & 60 & test & GPT4 Eval \\
% MultiDocVQA \citep{tito2023hierarchical} & UCSF-IDL & Document & Short Answer & 5019 / 5187 & test / val & ANLS / Accuracy \\
% NoCaps \citep{agrawal2019nocaps} & Open Images V4 dataset \citep{BASHIRI201871} & Novel Object Captioning & Short Answer & 4500 & val & CIDEr / SPICE / Bleu / Meteor / ROUGE \\
% OCRBench \citep{liu2023hidden} & Public Dataset & Text Recognition & Short Answer & 1000 & test & Exact Match \\
% OKVQA \citep{marino2019ok} & MSCOCO \citep{lin2014microsoft} & knowledge-based visual question answering & Short Answer & 5046 & val & Exact Match \\
% OlympiadBench \citep{he2024olympiadbench} & Public Dataset & Reasoning & Short Answer & 2126 / 6351 & test-en / test-cn & Exact Match \\
% POPE \citep{li2023evaluating} & MSCOCO \citep{lin2014microsoft} & Hallucination & Yes or No & 9000 & test & Accuracy / Precision / Recall / F1 / Yes Ratio \\
% Q-Bench ~\citep{wu2023q} & Internet & Image Quality Assessment & Short Answer & Muiti-Choice & 2990 & test & Exact Match / GPT4 Eval \\
% RealWorldQA ~\citep{grokv2024} & Internet & Real world scenarios QA & Muiti-Choice & 765 & test & Exact Match \\
% Refcoco \citep{kazemzadeh-etal-2014-referitgame, Mao_2016_CVPR} & Internet & Referring Expression & Short Answer & 5000, 1975, 1810, 8811 & bbox-test, bbox-testA, bbox-testB, bbox-val & CIDEr \\
% Refcoco \citep{kazemzadeh-etal-2014-referitgame, Mao_2016_CVPR} & Internet & Referring Expression & Short Answer & 5000, 1975, 1810, 8811 & seg-test, seg-testA, seg-testB, seg-val & CIDEr \\
% Refcoco+ \citep{kazemzadeh-etal-2014-referitgame, Mao_2016_CVPR} & Internet & Referring Expression & Short Answer & 1975, 1798, 3805, & bbox-testA, bbox-testB, bbox-val, & CIDEr \\
% Refcoco+ \citep{kazemzadeh-etal-2014-referitgame, Mao_2016_CVPR} & Internet & Referring Expression & Short Answer & 1975, 1798, 3805 & seg-testA, seg-testB, seg-val & CIDEr \\
% Refcocog \citep{kazemzadeh-etal-2014-referitgame, Mao_2016_CVPR} & Internet & Referring Expression & Short Answer & 5023, 7573, & bbox-testb, box-val, & CIDEr \\
% Refcocog \citep{kazemzadeh-etal-2014-referitgame, Mao_2016_CVPR} & Internet & Referring Expression & Short Answer & 5023, 7573 & seg-test, seg-val & CIDEr \\
% ScienceQA \citep{lu2022learn} & Internet (IXL Learning) & Science, World Knowledge, Reasoning & Muiti-Choice & 4241 & test & Exact Match \\
% ScreenSPOT~\citep{cheng2024seeclick} & Desktop & Mobile Apps GUI & GUI Understanding & Navigation & Short Answer & Coordinates & 1272 & test & CIDEr / IOU \\
% SEED-Bench \citep{li2023seed} & CC3M Dataset \citep{sharma2018conceptual} & Spatial and Temporal Understanding & Muiti-Choice & 17990 & test & Exact Match / Perplexity \\
% SEED-Bench-2 \citep{li2023seedbench2} & CC3M Dataset \citep{sharma2018conceptual} & Multi-task & Muiti-Choice & 24371 & test & Exact Match \\
% ST-VQA \citep{biten2019scene} & Public Dataset & Highlevel Semantic Information Understanding & Short Answer & 4070 & test & Submission \\
% SynthDoG \citep{kim2022donut} & Internet & Text Understanding & Free-form & 500 / 500 & val-en / val-zh & Tree Edit Distance \\
% TextCaps \citep{sidorov2019textcaps} & Open Images v3 \citep{krasin2017openimages} & Text Understanding & Captioning & 21953 / 3166 / 3289 & train / val / test & Bleu / METEOR / ROUGE_L / CIDEr / SPICE \\
% TextVQA \citep{singh2019towards} & Open Images v3 \citep{krasin2017openimages} & Text Understanding & Short Answer & 5000 / 5734 & val / test & Exact Match \\
% VisualWebBench~\citep{liu2024visualwebbench} & Webpages & Webpage Understanding & OCR & Reasoning & Short Answer & Muiti-Choice & 1536 & test & Exact Match / ROGUE_L / F1 \\
% VizwizVQA \citep{gurari2018vizwiz} & Public Dataset & Poor Quality Image Understanding & Short Answer & 8000 / 4319 & test / val & Exact Match \\
% VQAv2 \citep{balanced_vqa_v2} & COCO \citep{lin2014microsoft} & Visual Question Answering & Free-form & 447793 / 214354 & test / val & Exact Match \\
% WebSRC \citep{chen2021websrc} & SWDE \citep{hao2011one} & Self-Collected & Structure of Web Page & Short Answer & Yes or No & 40357 / 52826 & test / dev & Exact match / F1 / POS \\ \bottomrule
% \end{tabular}%
% }

==> tables/contamination_results.tex <==
\resizebox{0.98\textwidth}{!}{
\setlength{\tabcolsep}{12pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{lc|c|c}
    \toprule
    & & \multicolumn{1}{c|}{Image overlap (\%)} & \multicolumn{1}{c}{Text overlap (\%)} \\
    \cmidrule{3-4}
    Dataset & Split & LLaVA-NeXT Data & LLaVA-NeXT Data \\
    \midrule
    \multicolumn{4}{c}{\textit{Math \& Science}} \\
    \midrule
    AI2D~\citep{kembhavi2016diagram} & test & 6.09 & 25.97 \\
    MathVista~\citep{lu2024mathvista} & testmini & 9.90 & 7.70 \\
    ScienceQA~\citep{lu2022learn} & img & 0.35 & 1.54 \\
    \midrule
    \multicolumn{4}{c}{\textit{Doc \& Inforgraphic}} \\
    \midrule
    ChartQA~\citep{masry2022chartqa} & test & 68.64 & 26.52 \\
    DocVQA~\citep{mathew2020docvqa} & val & 36.08 & 4.06 \\
    InfoVQA~\citep{mathew2020docvqa} & test & 0.14 & 0.39 \\
    \midrule
    \multicolumn{4}{c}{\textit{Caption}} \\
    \midrule
    COCO2014~\citep{lin2015microsoft} & val & 46.05 & 22.19 \\
    Flickr30k~\citep{young-etal-2014-image} & test & 2.97 & 0.00 \\
    NoCaps~\citep{agrawal2019nocaps} & val & 2.53 & 19.98 \\
    TextCaps~\citep{sidorov2020textcaps} & val & 3.79 & 0.00 \\
    \midrule
    \multicolumn{4}{c}{\textit{VQA}} \\
    \midrule
    GQA~\citep{hudson2019gqa} & testdev-balanced & 13.91 & 9.50 \\
    TextVQA~\citep{singh2019vqa} & val & 3.90 & 2.00 \\
    VQAv2~\citep{balanced_vqa_v2} & val & 46.21 & 2.90 \\
    \midrule
    \multicolumn{4}{c}{\textit{Multi-task benchmark}} \\
    \midrule
    CMMMU \citep{zhang2024cmmmu} & val & 2.89 & 1.11 \\
    MMBench \citep{liu2024mmbench} & cn-dev & 2.77 & 0.81 \\
    MMBench \citep{liu2024mmbench} & en-dev & 2.77 & 7.97 \\
    MME \citep{fu2024mme} & test & 1.60 & 1.39 \\
    MMMU \citep{yue2023mmmu} & val & 2.67 & 3.56 \\
    MMVet \citep{yu2023mmvet} & val & 4.13 & 3.21 \\
    SEED-Bench \citep{li2023seedbench} & all & 1.11 & 13.84 \\
    \midrule
    \multicolumn{4}{c}{\textit{Others}} \\
    \midrule
    LLaVA-W \citep{liu2023visual} & test & 5.00 & 1.67 \\
    POPE \citep{li2023evaluating} & val & 42.20 & 0.00  \\
\bottomrule
\end{tabular}
}

==> tables/livebench_results.tex <==
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.2}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{@{}c|c|ccccc@{}}
\toprule
\textbf{Models} & \textbf{Overall Scores} & \textbf{Basic} & \textbf{Contextual} & \textbf{Deeper Impl.} & \textbf{Broader Impl.} & \textbf{Insights} \\ \midrule
Fuyu-8B          & 69.8 & 56.2 & 78.9 & 77.4 & 77.4 & 61.2 \\
Idefics-2-8B     & 45.9 & 53.6 & 42.7 & 42.3 & 47.0 & 33.7 \\
Claude-3-Haiku   & 47.8 & 57.0 & 44.8 & 41.1 & 44.5 & 39.1 \\
Claude-3-Sonnet  & 60.6 & 61.4 & 56.5 & 60.0 & 62.0 & 52.2 \\
LLaVA-1.5-7B     & 68.5 & 54.1 & 78.4 & 76.2 & 91.0 & 59.2 \\
Gemini-1.0-Pro   & 71.2 & 74.3 & 66.2 & 73.8 & 79.2 & 67.8 \\
LLaVA-1.5-13B    & 74.8 & 64.2 & 82.3 & 75.0 & 89.0 & 75.0 \\
Gemini-1.5-Flash &      &      &      &      &      &      \\
LLaVA-NeXT-72B   & 90.41 & 85.4 & 93.1 & 91.7 & 96.0 & 92.9 \\ \midrule
\textit{Best Human}       &         &  &  &  &  &  \\ \midrule
GPT-4V           & 90.5 & 90.1 & 94.0 & 83.9 & 95.5 & 87.5 \\
GPT-4O           & 94.4 & 91.9 & 96.6 & 92.3 & 96.5 & 94.6 \\ \bottomrule
\end{tabular}
}

==> tables/runtime_estimate.tex <==
\resizebox{\textwidth}{!}{
    \begin{tabular}{cc|ccccc}
    & & LLaVANeXT-vicuna-7B & LLaVANeXT-LLaMA-8B & LLaVANeXT-34B & LLaVANeXT-72B & LLaVANeXT-110B \\
    \midrule
    \multirow{2}{*}{Total Time (hrs)} & Full & 40 & 42 & 200 & 1200 & 1450 \\
    & Lite & 0.25 & 0.25 & 1 & 7.75 & 9 \\
    \end{tabular}
}
